ISSF: The Intelligent Security Service Framework for Cloud-Native Operation

The growing system complexity from microservice architectures and the bilateral enhancement of artificial intelligence (AI) for both attackers and defenders presents increasing security challenges for cloud-native operations. In particular, cloud-native operators require a holistic view of the dynamic security posture for the cloud-native environment from a defense aspect. Additionally, both attackers and defenders can adopt advanced AI technologies. This makes the dynamic interaction and benchmark among different intelligent offense and defense strategies more crucial. Hence, following the multi-agent deep reinforcement learning (RL) paradigm, this research develops an agent-based intelligent security service framework (ISSF) for cloud-native operation. It includes a dynamic access graph model to represent the cloud-native environment and an action model to represent offense and defense actions. Then we develop an approach to enable the training, publishing, and evaluating of intelligent security services using diverse deep RL algorithms and training strategies, facilitating their systematic development and benchmark. The experiments demonstrate that our framework can sufficiently model the security posture of a cloud-native system for defenders, effectively develop and quantitatively benchmark different services for both attackers and defenders and guide further service optimization.

==> related_work.tex <==
% 云原生、云原生应用、云原生可扩展性
\cite{henning2022configurable}
Following the rise of cloud computing as preferred deployment infrastructure for many applications, we are now witnessing how large-scale software systems are increasingly being designed as “cloud-native” applications (Gannon et al. 2017; Kratzke and Quint 2017). Under the umbrella term “cloud-native”, a wide range of tools and patterns emerged for simplifying, accelerating, and securing the development and operation of software systems in the cloud. Key concepts are containers, dynamic orchestration, and microservices, which provide a new level of hardware abstraction, while still providing a high flexibility regarding the system’s deployment. An entire ecosystem of such tools has grown in recent years under the umbrella of the Cloud Native Computing Foundation,1 a suborganization within the Linux Foundation. Most prominent among these tools is probably Kubernetes (Burns et al. 2016), which has become the de-facto standard orchestration tool for cloud-native applications. Nowadays, all major cloud providers offer managed Kubernetes clusters. With such offerings, users only specify the desired cluster size (e.g., number of virtual or physical nodes and properties of nodes). For the actual operation of their applications (e.g., scaling, updating, or repairing), they only interact with the Kubernetes API. Recently, a further level of abstraction can be observed. For example, the Google Cloud Platform launched its Kubernetes Autopilot in 2021, which adjusts underlying node pools based on the current demand and only charges users for the containers they actually deploy.

A definition of the term “cloud-native” is provided by the Cloud Native Computing Foundation, which states that “cloud native technologies empower organizations to build and run scalable applications in modern, dynamic environments such as public, private, and hybrid clouds” (Cloud Native Computing Foundation 2018). This definition already includes the requirement for scalability. Similarly, microservice architectures (a common pattern for cloud-native applications (Balalaie et al. 2016)) are often adopted to cope with scalability requirements (Kratzke and Quint 2017; Soldani et al. 2018; Knoche and Hasselbring 2019). However, although scalability is often named as a crucial motivation for adopting cloudnative architectures or deployments, research is lacking a commonly accepted method to empirically assess and compare the scalability of cloud-native applications.

A software system can be considered scalable within a certain load intensity range if for all load intensities within that range it is able to meet its service level objectives, potentially by using additional resources. Both load intensity and provisioned resources can be evaluated with respect to different dimensions. Typical load dimensions are, for example, the amount of concurrent users or number of requests, while resources are often varied in the number of processing instances or equipment of the individual instances. This understanding of scalability (albeit less formally) is shared by textbooks addressed to practitioners (Kleppmann 2017; Gorton 2022).

Another quality that is often used in cloud computing is elasticity (Lehrig et al. 2015). Scalability and elasticity are related, but elasticity takes temporal aspects into account and describes how fast and how precisely a system adapts its provided resources to changing load intensities (Herbst et al. 2013; Islam et al. 2012). Scalability, on the other hand, is a prerequisite for elasticity, but is a time-free notion describing whether increasing load intensities can be handled eventually

\cite{li2023fisc}
Many applications, such as data analytics [1], machine learning [2], and transactional workflows [3, 4] are deployed in public clouds. The emerging cloud-native technologies are shifting virtualization in clouds from virtual machines (VM) to containers and pushing up the abstraction provided to tenants from resources (e.g., CPU and memory) to services (e.g., database and object storage service). As such, cloud service providers (CSPs) must rethink their fundamental services to provide efficient, flexible support to cloud-native applications.

With the development of cloud-native technology (e.g., microservice, container, and serverless computing), more and more tenants are deploying their applications into the public cloud and directly using the services provided by CSPs (e.g., database and object storage service). In 2020, Alibaba also migrated all its core businesses, such as Taobao and Tmall, to cloud-native containers. Cloud-native technologies substantially simplify the development and operation of tenants and demonstrate two characteristics. First, with fine-grained containers being used instead of VMs, the number of containers in a computation server can exceed 1000 [17, 18], i.e., ∼10 times more than that of VMs. Second, cloud-native technologies push up the abstraction provided to tenants from VMs to services. The implementation of services is transparent to tenants but must provide high performance under heterogeneous workloads. To this end, bare-metal DPUs are increasingly used to accelerate cloud-native applications. For example, AWS adopts Nitro [19] and Alibaba adopts X-Dragon [20,21]. These bare-metal DPUs utilize the virtio technology for I/O virtualization and can provide high-performance support to a broad range of cloud services.

\cite{jin2019dseom}
As a lightweight alternative to the virtual machine (VM) in conventional cloud infrastructures, container has shorter startup time and lower virtualization overhead [1]. Moreover, container also provides a consistent and portable software environment, which can make cloud services ignore the difference between platforms to easily run and scale anywhere. Because of the proven benefits, container further boosts the rapid development of microservice architecture which has been widely applied in many companies, such as Uber and Netflix etc. [2], [3]. In the microservice architecture, a monolithic application is decoupled into a set of independent microservices performing a single function. It can help service providers simplify the process of updating, scheduling and scaling service [4]. At the same time, the microservice architecture has better modularity and enables application developers to take advantage of services from other providers.

Based on lightweight (OS-level) virtualization, container needs less system resources to run a service and has faster startup times, superior performance of I/O throughput and lower latency compared with VM [15]. At the same time, by packaging application code and dependencies together, container management platforms (such as Docker [16] and Kubernetes [17]) can provide a consistent environment for development, testing, and production of applications, which can shorten the release and update cycles greatly. Due to these characteristics, container can run in any cloud environments regardless of the differences between environments.

The aforementioned characteristics promote development of a new service architecture, microservice architecture [18], where the application is decoupled into a set of simple functional services called microservice. Each microservice serves as a single purpose, and is deployed in the container. In the cloud environment, a set of microservices interact with each other using HTTP or RPC to form a service chain and provide an integrated function to users. Incorporating features of the container mentioned above, the applying of microservice enables the cloud services to flexibly scale, deploy and schedule. However, it also extremely increases the dynamism of cloud environments since the microservice may be independently updated 10-100 times a day [6].

% 云原生安全
\cite{jin2019dseom}
Given the ever-expanding usage of container technology and microservice architecture, one of the biggest concern is whether the changes brought by them would affect the security of cloud environment. Different from the rigid VM-based cloud environment [5], microservice architecture makes service scaling and updating more flexible. And the update frequency of each service can be as high as hundreds of times a day [6]. However, the flexibility of microservices also causes the dynamism and complexity of cloud environment to increase tremendously, and meanwhile, may introduce some new security issues unintentionally. Specifically, due to the high-frequency update, defense mechanisms with fixed strategies may hardly cover the attack surface persistently in this dynamic environment. Thus, the effectiveness of defense mechanism would fluctuate (either increase or decrease) over time, which we call the effectiveness drift problem. Particularly, the drift problem is acute in proactive defense mechanism because its effectiveness highly depends on current situation of defense targets. If the defense strategies don’t match the supposed condition, the proactive defense mechanism may not work well.

Consequently, we focus on Moving Target Defense (MTD), a representative proactive defense mechanism, as the study subject in our work. MTD can continuously transform the attack surface of target system, such as randomizing execution environment [7], software implementation [8], and network topology [9] etc., to reduce the opportunity of the attack surface being exploited by attackers [10], [11]. Currently, to maximize the effectiveness of MTD, existing studies work on evaluating and optimizing implementation strategies of MTD [12], [13], [14]. However, these methods focus on the static deployment scenarios and can’t meet the requirements of dynamically optimizing MTD strategies in the container-based cloud environment. In this paper, we propose a framework called DSEOM to study and solve these problems mentioned above. As far as we know, DSEOM is the first framework for dynamically evaluating and optimizing the effectiveness of MTD techniques in the containerbased cloud environment at real time.

Different from traditional cloud environments, container technology and microservice architecture make up the container-based cloud environment. However, excepting for the advantages brought to container-based cloud environment, some security issues introduced by these new technologies are also being widely concerned. The main security issues include the weak isolation problem among containers [19] which also exists in VM-based cloud environment [20], greater attack surface caused by microservice [21], [22], and the security drift problem caused by its high dynamic [23].



% previous
\cite{zeng2023full}
In recent years, with the evolution of technologies for software development, operation, and maintenance, cloud-native architecture has grown in popularity owing to its unique features,
including lightweight virtualization, resource isolation, and management abilities. A recent study shows that more than 65\% of enterprises are embracing cloud-native technology to build their applications (Why make the transition to cloud native for your enterprise, 2021). One of the key components of the cloud-native system is containers. As the minimum viable functional unit for product integration and delivery, containers allow developers to concentrate on coding rather than software building and shipping following DevOps practices.

Other components including container orchestrator and service mesh also form the baseline of cloud-native infrastructure for supporting better virtualization and scalability. First, container orchestration allows cloud-native service providers to define how multiple containers are configured, deployed, monitored, and dynamically controlled in the platforms (Casalicchio, 2019). Second, the service mesh is proposed dedicatedly for fast, secure, and reliable communications among microservices. The most popular implementations of these two components are Kubernetes and Istio.



\cite{  }
One of the main research areas in moving target defense is to model interactions between the adversaries and the defenders. In the area of game-theoretic models for moving target defense, the most closely related work is from Prakash et al. [22], which introduces the model that our work uses. This model can also be used for defense against DDoS attacks [31], and defense for web applications [25]. Further, in this area, researchers have proposed MTD game models based on Stackelberg games [13], Markov Games [12,28], Markov Decision Process [32], and FlipIt game [20]. For solving a game model (i.e., finding the optimal playing strategies), numerous approaches such as solving a min-max problem [13], non-linear programming [12], Bellman equation [28,32], Bayesian belief networks [2], and reinforcement learning [9,20] has been suggested.


\cite{  }Application of machine learning—especially deep reinforcement learning (DRL)—for cybersecurity has gained attention recently. Nguyen et al. [19] surveyed current literature on applications of DRL on cybersecurity. These applications include: DRL-based security methods for cyber-physical systems, autonomous intrusion detection techniques [10], and multi-agent DRL-based game-theoretic simulations for defense strategies against cyber attacks.
For example, Malialis [14,15] applied multi-agent deep reinforcement learning on network routers to throttle the processing rate in order to prevent distributed denial of service (DDoS) attacks. Bhosale et al. [3] proposed a cooperative multiagent reinforcement learning for intelligent systems [7] to enable quick responses. Another example for multi-agent reinforcement learning is the fuzzy Q-Learning approach for detecting and preventing intrusions in wireless sensor networks (WSN) [26]. Furthermore, Tong et al. [29] proposed a multi-agent reinforcement learning framework for alert correlation based on double oracles.

\cite{zhang2022optimal}
Attack graph (AG) is commonly used to represent a space of sequential attacks for finding the attack paths against a specific network. A large body of the literature on attack graphs focuses on how to represent and analyze complex security scenarios. Ritchey et al. [8] use AG to search if there exists a series of attacks that could lead to network compromise. Barik et al. [5] present a consolidated view of major attack graph generation and analysis techniques, aiming to patch networks by computing a minimal set of vulnerabilities. In [7], the authors introduce Bayesian attack graphs, which combines attack graphs with quantified uncertainty on attack states and relations. The integration of attack graph and game-theory is also a research hotspot. In [9], the authors propose a gametheoretic model to detect and mitigate attacks by deploying deceptive hosts and services. In [10], Letchford et al. present a Stackelberg game model of security, where the the attacker chooses an optimal attack plan that circumvents the deployed mitigation and the defender decides which vulnerabilities to fix in the attack graph to mitigate the loss. In [11], the authors propose a game-theory based algorithm to compute strategies and develop a reinforcement learning based method for the attacker to determine when to stop. The most closely related prior work is perhaps [12], which presents a simulation-based approach to analyze the attacker and defender by a set of heuristic strategies. In contrast, we us deep reinforcement learning to compute the strategies.

\cite{zhang2022optimal}
Attack graph (AG) is commonly used to represent a space of sequential attacks for finding the attack paths against a specific network. A large body of the literature on attack graphs focuses on how to represent and analyze complex security scenarios. Ritchey et al. [8] use AG to search if there exists a series of attacks that could lead to network compromise. Barik et al. [5] present a consolidated view of major attack graph generation and analysis techniques, aiming to patch networks by computing a minimal set of vulnerabilities. In [7], the authors introduce Bayesian attack graphs, which combines attack graphs with quantified uncertainty on attack states and relations. The integration of attack graph and game-theory is also a research hotspot. In [9], the authors propose a gametheoretic model to detect and mitigate attacks by deploying deceptive hosts and services. In [10], Letchford et al. present a Stackelberg game model of security, where the the attacker chooses an optimal attack plan that circumvents the deployed mitigation and the defender decides which vulnerabilities to fix in the attack graph to mitigate the loss. In [11], the authors propose a game-theory based algorithm to compute strategies and develop a reinforcement learning based method for the attacker to determine when to stop. The most closely related prior work is perhaps [12], which presents a simulation-based approach to analyze the attacker and defender by a set of heuristic strategies. In contrast, we us deep reinforcement learning to compute the strategies.

\cite{9407888}
However, such game problem still faces the challenge of acquiring the equilibrium in a huge game space. A more effective way of this challenge is to train a growing population of player strategies and use heuristic methods to guide the population evolution [9]. The ever-increasing popularity of artificial intelligence (AI) offers a new perspective to guide the population evolution. By combining the deep learning (DL) and reinforcement learning (RL), deep reinforcement learning (DRL) [10] has a strong ability to explore new strategies through value based or policy based approaches. Some researches [11], [12] have studied the AI-aided attackdefense confrontation game in different scenarios. However, there still exist research gaps at the network abstraction and modeling. Previous work only focuses on the confrontation game on random networks, while scale-free networks also need an urgent enhancement at defense performance, perhaps via the AI-aided methods. Random graph, as a network abstraction, can model a part of network systems. Different from the random network, the scale-free network is more vulnerable to potential targeted attacks, which makes it more urgent to enhance the security of the scale-free network. It remains an open problem that whether the AI-aided game can achieve a better performance in scale-free networks than that in random networks.

\cite{chen2022gpds}
To defend against interference attacks, the common technical means of wireless networks include power control (Feng and Haykin, 2019), beamforming (Tang, Wang, Zhang, Chu, and Han, 2021), relay assistance (Yang et al., 2020), and frequency hopping (Shi, An, and Li, 2021). In traditional wireless networks, power control is a powerful anti-interference strategy. Specifically, the wireless network system can use game theory to obtain the optimal anti-interference power control strategy of the devices and improve the transmission rate (Chen, Song, Xin, & Backens, 2013; Lv et al., 2017). In addition, the trusted relay is also considered to be one of the promising anti-interference technologies. Wireless networks can reduce the channel interference of jammers through beamforming and relay selection (Hoang, Duong, Suraweera, Tellambura, and Poor, 2015).

However, many previous studies focus on the single agent antiinterference scenario, and do not fully consider the possibility of mobile device cooperation in anti-jamming. With the development of multiagent technology, many anti-jamming studies have extended them works to multi-user scenarios (Elleuch, Pourranjbar, & Kaddoum, 2021; Yin et al., 2022). Because the previous defense technology is a passive and lagging defense means according to the configuration of attack characteristics and the issuance of defense strategies, the defense side is at a disadvantage in the anti-interference confrontation. Multi-user security Game represents the relationship between cooperation and competition among multiple users by extending the Markov game framework, so as to achieve multi-user cooperation and antiinterference to improve network security. Surprisingly, multi-agent reinforcement learning technology can realize the optimal attack and defense game in an incomplete information environment (Rowland et al., 2019; Torreño, Onaindia, & Sapena, 2015). In addition, the high-dimensional channel state and action space will slow down the training speed. Therefore, we propose a frequency hopping strategy based on multi-user anti-interference game. A deterministic gradient reinforcement learning algorithm is designed to obtain the optimal frequency hopping strategy of mobile devices in the worst case.

\cite{li2021understanding}
Security Monitor is a tactic applied by four reviewed studies to detect attacks of microservice instances. Motivation MSA introduced many security challenges to be addressed. One concern is that it uses distributed methods to communicate amongst participating microservices, whose network/infrastructure complexity may be exploited by attackers and cause the burden of detecting attacks [Sun 15, Tork 17]. Another concern is the lack of enough trust on specific microservices or among distributed microservices, since one microservice may be compromised and controlled by an adversary abusing its privileges. Therefore, a tactic is needed to flexibly monitor risky aspects of microservices or their Infrastructure and enforce policies on them in order to detect or prevent both external and internal threats targeting MSA applications.

Authentication and Authorization is tactic to resist attacks in MSA and applied by four studies. Authentication is a process by which to confirm the identity a user or a party and authorization is a mechanism by which a principal is mapped to the action allowing an identity to do.

Constraints for those above solutions of Authentication and authorization tactic are: 1) Key exchange may requires the key management and moves the focus of trust from a small amount of sound and cryptographical protocols to various unspecified mechanisms. The adoption of this approach lead to the trade-offs between performance and security. 2) TLS-based client certificates are not used very frequently and support should be explicitly invoked by the application code, since this method does not have strict mandate on the use and validation of certificates. Furthermore, it may be insufficient to carry out the authentication only based on host name. 3) Deploying de and integrating trusted third parties that allow federated security is very complex and requires specialized knowledge.

\cite{zeng2023full}
We collect the vulnerabilities of Docker components from the CVE Details database (CVE Details, 2022), which enables us to browse all the CVEs related to a specific software vendor, i.e., Docker (2022), containerd (Containerd Security Vulnerabilities, 2022), and runc (Runc Security Vulnerabilities, 2022). We focus on the vulnerabilities from 2017 to 2022, and exclude the ones that are specific to a Linux distribution or related to Docker images, only caring about the crucial components needed to run and manage containers. As shown in Table 1, from the “Components” dimension, Docker is the most vulnerable component, accounting for more than 50\% of vulnerabilities. From the “Attack Enabled” dimension, it is depicted that over 80\% of the vulnerabilities can cause privilege escalation.

Container Security Analysis. Lin et al. focus on detecting security attacks using a distributed learning framework with insuffi- cient training data in containerized applications (Lin et al., 2020). Shu et al. create a scalable Docker image vulnerability analysis (DIVA) framework to find vulnerabilities in images on Docker Hub (Shu et al., 2017). Wong et al. performed threat modeling on the container ecosystem using the STRIDE threat modeling framework (Wong et al., 2021). Combe et al. studied the security challenges brought by Docker (Combe et al., 2016). Martin et al. studied the vulnerabilities of the Docker ecosystem (Martin et al., 2018). Lin et al. measured the security implication of containers (Lin et al., 2018). Sultan et al. provided an overall survey of container security (Sultan et al., 2019). Wist et al. analyzed vulnerabilities of docker hub images Wist et al. (2021). On reducing the attack surface and detecting attacks on containers, Lic-Sec (Zhu and Gehrmann, 2021) provided an Apparmor profile generation method using dynamic analysis to reduce the container attack surface, while Confine Ghavamnia et al. (2020) achieve a similar goal using static analysis. Jian and Chen (2017) proposed a method for detecting kernelbased container escape attacks. gVisor (2022), kata (Randazzo and Tinnirello, 2019) and Firecracker (Agache et al., 2020) enhanced the isolation mechanism using sandbox or light VM technology. Though being more secure, these approaches can cause more performance overhead. The comparison between these different container runtimes has also been studied (Debab and Hidouci, 2020; Flauzac et al., 2020; Mavridis and Karatza, 2021).

CNI Security Analysis. A comparison between different CNI plugins is provided (Qi et al., 2021). This paper is an assessment of CNIs performance, describing each CNI plugin in detail. However, it does not analyze the security problems the CNIs may cause. Minna et al. (2021) focus on the security implications of Kubernetes networking. The authors propose that there are unexpected attacks that happened in Kubernetes networking. They introduce the network architecture and give attack scenarios but they don’t find all CVEs related to the scenario. Nam et al. conduct security of container network and present a security enforcement network stack (Nam et al., 2020). They mainly focus on how to improve the performance and security of container networks. But they don’t evaluate the CVEs on their prototype. Our paper presents an overview of CNIs architecture and focuses on vulnerability analysis

\cite{zdun2023microservice}
Microservice architectures [29, 33, 48] structure an application as a collection of autonomous services. They have a set of important tenets such as development in independent teams, polyglot technology stacks including polyglot persistence and programming languages, cloud-native technologies and architectures, use of lightweight containers, loosely coupled service dependencies, high releasability, end-to-end tracing and monitoring, and continuous delivery [29, 33, 62]. This article focuses on the security aspects of microservice architectures. Despite numerous published guidelines and best practices [8, 34, 37], the architecture of microservice systems is challenging with regard to security. This is due to the size and complexity of microservice systems, their polyglot nature, and the need for continuous evolution and frequent release of these systems. In this context, manually validating whether security features are used as intended throughout the system is a time-consuming and error-prone task. For architecturally relevant security features, architectural abstraction can help focus only on the relevant aspects, but still substantial effort is required e.g., to check a large-scale system’s architecture for conformance to security tactics.
